Learning to be a Statistician: Learned Estimator for Number of Distinct Values

Estimating the number of distinct values (NDV) in a column is useful for many tasks in database systems, such as columnstore compression and data profiling. In this work, we focus on how to derive accurate NDV estimations from random (online/offline) samples. Such efficient estimation is critical for tasks where it is prohibitive to scan the data even once. Existing sample-based estimators typically rely on heuristics or assumptions and do not have robust performance across different datasets as the assumptions on data can easily break. On the other hand, deriving an estimator from a principled formulation such as maximum likelihood estimation is very challenging due to the complex structure of the formulation. We propose to formulate the NDV estimation task in a supervised learning framework, and aim to learn a model as the estimator. To this end, we need to answer several questions: i) how to make the learned model workload agnostic; ii) how to obtain training data; iii) how to perform model training. We derive conditions of the learning framework under which the learned model is workload agnostic, in the sense that the model/estimator can be trained with synthetically generated training data, and then deployed into any data warehouse simply as, e.g., user-defined functions (UDFs), to offer efficient (within microseconds on CPU) and accurate NDV estimations for unseen tables and workloads. We compare the learned estimator with the state-of-the-art sample-based estimators on nine real-world datasets to demonstrate its superior estimation accuracy. We publish our code for training data generation, model training, and the learned estimator online for reproducibility.

==> paper-related.tex <==
%!TEX root = paper.tex

\section{Related work}
\noindent\textbf{Sketch based NDV estimation.} Sketch based methods (e.g. Hyperloglog~\cite{flajolet2007hyperloglog}) scan the entire dataset once and keep a sketch that is used to estimate NDV. These methods are very accurate but requires to examine the entire dataset. 
In contrast, our method only needs a very small sample, so our method is advantageous when the dataset is extremely big or when some data points are not accessible.

\noindent\textbf{Sampling based NDV estimation.} There are many sampling based estimators in literature. The only unbiased estimator is the Goodman's estimator~\cite{goodman1949estimation}, which is unusable in practice due to its extremely high variance and numerical instability~\cite{haas1995sampling}. The only estimator with guaranteed error bound is the GEE estimator, which is constructed based on the heuristic to balance two extreme NDV bounds with use geometric mean~\cite{charikar2000towards}. Various estimators are derived by making different assumptions: infinite population size~\cite{chao1992estimating}, certain condition of skewness of the data distribution~\cite{shlosser1981estimation}, power-law or Zipfian data distribution~\cite{motwani2006distinct}. There are also hybrid estimators that use different base estimators according to data properties like skewness to combine the strength of different estimators~\cite{haas1995sampling,charikar2000towards}. In sum, existing estimators are mostly based on heuristics or assumptions. In contrast, our method follows the principle of maximum likelihood estimation. %Naively use maximum likelihood estimation is of exponential complexity for estimating NDV, so we instead learn a model to approximate the functional form of maximum likelihood estimation.

\noindent\textbf{Learned Cardinality Estimation.} There are works that learn a model to estimate cardinality or selectivity of a query~\cite{anagnostopoulos2015learning, lakshmi1998selectivity, liu2015cardinality, 
dutt2019selectivity,
kipf2018learned}. All of them follow the same paradigm: the query is used as the primary feature and training data comes from the records of previous query executions. These methods require executing a huge number of queries to obtain enough training data~\cite{wang2020we}. In dynamic environments, these methods are very fragile and typically require huge efforts of retraining~\cite{wang2020we}. Although we also learn a model to estimate NDV/cardinality, our method is totally different from previous learning based methods. Our method learns to estimate NDV from a small sample but not a query so we use features from the sample instead of the query. In addition, our method is workload agnostic so it is very robust in dynamic environments.


